Sampling Methods for Inner Product Sketching

Recently, Bessa et al. (PODS 2023) showed that sketches based on coordinated weighted sampling theoretically and empirically outperform popular linear sketching methods like Johnson-Lindentrauss projection and CountSketch for the ubiquitous problem of inner product estimation. We further develop this finding by introducing and analyzing two alternative sampling-based methods. In contrast to the computationally expensive algorithm in Bessa et al., our methods run in linear time (to compute the sketch) and perform better in practice, significantly beating linear sketching on a variety of tasks. For example, they provide state-of-the-art results for estimating the correlation between columns in unjoined tables, a problem that we show how to reduce to inner product estimation in a black-box way. While based on known sampling techniques (threshold and priority sampling) we introduce significant new theoretical analysis to prove approximation guarantees for our methods.

==> kmv.tex <==


In this work, we propose a customized approach for the problem setting using Weighted MinHash as a reference. Weighted MinHash, originally proposed in \cite{BessaDFMMSZ:2023}, is a method that addresses the issue of unbounded vector entries by scaling and discretizing them. We adopt the Weighted MinHash approach to our problem setting by using a similar process to construct the KMV sketch.

To carry out the KMV sketch, we use a random hashing function $h\left\{1,2,...,n \right\} \rightarrow \left [0,1 \right]$ and store the $K$ minimum hash values. 

We describe the customized approach in three steps: First, we normalize the vector by dividing each entry by its $\ell_2$ norm and add the norm as a single scalar to the sketch. Second, we assume that the squared entries of the normalized vector are integer multiples of some small value $p \ll 1$. We then construct an "expanded" vector with entries set such that the first $\tilde{a}_i^2/p$ entries in each block of $1/p$ indices are 1 and the rest are 0. Finally, we compute the KMV sketch by storing the $K$ minimum hash values of the expanded vector.

The KMV approach provides a practical solution that guarantees accurate results. We analyze the variance and expected value of the estimator and show that it achieves the desired properties.

Let's denote $U^{hash}_i{(a)}$ as the $i^\text{th}$ minimum hash value of $h(\bar{a})$, and $U^{val}_i{(a)}$ as the corresponding value of $\tilde{a}$ to $U^{hash}_i{(a)}$.

Suppose that $U^{hash}{(a)}$ denotes the set of $k$ distinct hash values of $a$. Let $U^{hash}{(a\cup b)}$ be a set that contains the smallest $k$ values from $U^{hash}{(a)}$ and $U^{hash}{(b)}$.

Similarly to the union case, we can use the same procedure over the intersection of two sets. We define our weighted KMV as follows:

\begin{align*}
WKMV(a,b) &= \left| a \right|\left| b \right| \cdot \frac{k-1}{k \cdot U^{hash}_k(a\cup b)} \cdot \\
& \qquad \sum_{i=1}^{k}\sum_{j=1}^{k} \mathbbm{1} \left [ U^{hash}_i(a) = U^{hash}_j(b) \in U^{hash}(a\cup b) \right ] \cdot \\
& \qquad \qquad \frac{U^{val}_i(a) \cdot U^{val}_j(b)}{min(U^{val}_i(a),U^{val}_j(b))^2}
\end{align*}

Denote $M = \sum_{t \in A\cup B}^{} max(\tilde{a}_t^2,\tilde{b}_t^2)$. We note that a random variable $Z{i,j}$ follows a Bernoulli distribution since it takes a value of $\frac{\tilde{a}_i \tilde{b}_i}{min(\tilde{a}_i,\tilde{b}_i)^2}$ if the corresponding objects appear in the $k$ minimum hash values, which happens with probability $\frac{k}{M}$.

\begin{align*}
Z_{i,j} = \begin{cases}
\frac{\tilde{a}_i \tilde{b}_i}{min(\tilde{a}_i,\tilde{b}_i)^2} \quad\quad \text{ with probability } \frac{k}{M}\\
0 \qquad\qquad\qquad\text{ with probability } 1 - \frac{k}{M}
\end{cases}
\end{align*}

Therefore, using this estimator, we can compute the expected value as precisely the inner product of the two original vectors $a$ and $b$.

\begin{align*}
\E[WKMV(a,b)] &= \left| a \right|\left| b \right| \cdot \E\left[\frac{k-1}{k \cdot U^{hash}_{k}(a\cup b)}\right] \cdot \\ \sum_{i\in A \cap B } \sum_{j \in min(\tilde{a}i,\tilde{b}i)^2 } \E\left[Z{i,j}\right]
&= \left| a \right|\left| b \right| \cdot \E\left[\frac{k-1}{k \cdot U^{hash}_{k}(a\cup b)}\right] \cdot \\ \sum_{i\in A \cap B } \sum_{j \in min(\tilde{a}_i,\tilde{b}_i)^2 } \frac{k \cdot \tilde{a}_i \tilde{b}_i}{min(\tilde{a}_i, \tilde{b}_i)^2\cdot M}
&= \left| a \right|\left| b \right| \cdot \E\left[\frac{k-1}{k \cdot U^{hash}_{k}(a\cup b)}\right] \cdot\\ \sum_{i\in A \cap B } \frac{k \cdot \tilde{a}_i \tilde{b}_i}{M} \
&= \left| a \right|\left| b \right| \cdot \frac{M}{k} \cdot \frac{k}{M}\cdot \langle \tilde{a},\tilde{b}\rangle = \langle a,b\rangle
\end{align*}

==> vector-example-Limbo.tex <==
\begin{figure}[t]
\centering
\footnotesize
\parbox{1.0\linewidth}{
\centering
\setlength{\tabcolsep}{0.35em}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\multicolumn{10}{c}{}        \\
    \hline
    index & \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 & \bf 6 & \bf 7 & \bf 8 & \bf 9 & \bf 10 & \bf 11 & \bf 12 & \bf 13 & \bf 14 & \bf 15 & \bf 16 \\
    \hline
    $\bv a$ & 0 & 0 & 1.5 & 0 & 0 & 2.3 & 0 & -5 & 0 & 0 & 0.5 & 0 & 3 & 0 & 0 & -3.7\\
    \hline
    $\bv b$ & 0 & -2 & -3.1 & 0 & 0 & 0 & 0.4 & -4.2 & 0 & 1.5 & 1 & 0 & 3 & -5.9 & 0 & 0\\
    \hline
\end{tabular}
}
\vspace{-1em}

\caption{
Vectors $\bv{a}$ and $\bv{b}$ to be sketched. We can calculate the exact value of $\langle \bv a, \bv b\rangle = 25.85$.
}
\vspace{-1em}
\label{fig:ex-vectors}
\end{figure}


